Pushing the Limits of Simple Pipelines for Few-Shot Learning: External Data and Fine-Tuning Make a Difference

Few-shot learning (FSL) is an important and topical problem in computer vision that has motivated extensive research into numerous methods spanning from sophisticated meta-learning methods to simple transfer learning baselines. We seek to push the limits of a simple-but-effective pipeline for more realistic and practical settings of few-shot image classification. To this end, we explore few-shot learning from the perspective of neural network architecture, as well as a three stage pipeline of network updates under different data supplies, where unsupervised external data is considered for pre-training, base categories are used to simulate few-shot tasks for meta-training, and the scarcely labelled data of an novel task is taken for fine-tuning. We investigate questions such as: (1) How pre-training on external data benefits FSL? (2) How state-of-the-art transformer architectures can be exploited? and (3) How fine-tuning mitigates domain shift? Ultimately, we show that a simple transformer-based pipeline yields surprisingly good performance on standard benchmarks such as Mini-ImageNet, CIFAR-FS, CDFSL and Meta-Dataset. Our code and demo are available at https://hushell.github.io/pmf.

==> fig/overview.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1.0\columnwidth]{fig/pipeline_fig.pdf}
%\hfill
%\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\caption{
% 
    \textbf{Overview -- } A schematic of the simple-but-effective pipeline that we consider: \ourNameLong (\ourName). Following the red arrows, the pipeline turns a class-agnostic feature backbone into a generic feature backbone and ultimately a task-specific feature backbone. 
}
\label{fig:overview}
\end{figure}

% \begin{figure*}
% \begin{center}
% \includegraphics[width=.75\textwidth]{fig/pipeline_fig.pdf}
% %\hfill
% %\includegraphics[width=.99\columnwidth]{example-image-golden}
% \end{center}
% \caption{
% % 
% \textbf{Overview -- }
% A schematic of the simple pre-training, meta-training, fine-tuning pipeline that we consider. Following the red arrows, which indicate the information flow directions, we see how the pipeline turns a pre-trained feature backbone into a task-specific one. 
% }
% \label{fig:overview}
% \end{figure*}


==> fig/q1_q2.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=0.95\linewidth]{fig/pt_md.pdf}
\end{center}
\caption{
Comparison between self-supervised pre-training and supervised pre-training. To answer Q1 and Q2.
}
\label{fig:pt_md}
\end{figure}

==> fig/q3_q4.tex <==
\begin{figure}[ht]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
%\includegraphics[width=0.95\linewidth]{fig/pt_md_ft_dinosmall_lr1e-4.pdf}
\includegraphics[width=0.95\linewidth]{fig/fig3.pdf}
\end{center}
\caption{The impact of fine-tuning during meta-test on Meta-Dataset. Held out datasets such as Signs and COCO benefit from fine-tuning; as do those very different from ImageNet such as omniglot and QuickDraw.
%How do meta-training and fine-tuning affect the performance? Messages: 1) ViT backbones are able to extract good features for multiple domains, but they are not able to generalize well to unseen domains; 2) Fine-tuning yields similar performance no matter if meta-training was performed on single domain or multile domains. To answer Q3 and Q4.
}
\label{fig:pt_md}
\end{figure}

==> fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
%\includegraphics[width=\linewidth]{fig/boxplot_m-inet.pdf}
\includegraphics[width=\linewidth]{fig/fig1_clip.pdf}
\end{center}
\caption{
%\textbf{Teaser} -- 5 years of FSL research progress since Vinyals et al's 2016 study \cite{vinyals2016matching},  as measured by miniImageNet 5W5S accuracy. Backbone architecture has a substantial impact. %By simply substituting the backbone of ProtoNet to a self-supervised ViT (pre-trained with external data), the performance is significantly better than all prior work.
\textbf{How does pre-training and architecture affect few-shot learning?} 
Learning from a few shots can be achieved by a) meta-learning \cite{vinyals2016matching,zhang2021metaQDA} and b) transfer learning from self-supervised foundation models pre-trained on large-scale external data \cite{chen2020bigSimCLRV2,radford2021learning}. While the majority of FSL community focuses on the former, we show that the latter can be more effective because it enables the use of stronger architectures such as vision transformer (ViT) \cite{dosovitskiy2021imageTransformerVIT} -- and can be combined with simple meta-learners such as ProtoNet. The figure shows results aggregated from dozens of studies from the past 5 years of FSL research and the result of ProtoNet + ViT backbone + contrastive language-image pretraining (CLIP) \cite{radford2021learning} (yellow star). To emphasize the importance of pre-training, ProtoNet + randomly initialized ViT (blue square) is also compared.  
%in terms of miniImageNet (5-way-5-shot) performance. 
%which yields surprisingly good performance (on Mini-ImageNet and CIFAR-FS, 5-way-5-shot) comparing to the 5 years of FSL research progress since Vinyals et al's 2016 study \cite{vinyals2016matching}.
}
\label{fig:teaser}
\end{figure}

==> tab/cdfsl.tex <==
\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{l|lll|lll|lll|lll} 
\hline
\multirow{2}{*}{}       & \multicolumn{3}{c|}{ChestX} & \multicolumn{3}{c|}{ISIC} & \multicolumn{3}{c|}{EuroSAT} & \multicolumn{3}{c}{CropDisease}  \\ 
\cline{2-13}
                        & 5w5s  & 5w20s & 5w50s       & 5w5s  & 5w20s & 5w50s     & 5w5s  & 5w20s & 5w50s        & 5w5s  & 5w20s & 5w50s            \\ 
\hline
ProtoNet  \cite{snell2017prototypical} (RN10)  & 24.05 & 28.21 & 29.32       & 39.57 & 49.50  & 51.99     & 73.29 & 82.27 & 80.48        & 79.72 & 88.15 & 90.81            \\
RelationNet  \cite{sung2018relationNet} (RN10)           & 22.96 & 26.63 & 28.45       & 39.41 & 41.77 & 49.32     & 61.31 & 74.43 & 74.91        & 68.99 & 80.45 & 85.08            \\
MetaOptNet  \cite{lee2019meta}  (RN10)     & 22.53 & 25.53 & 29.35       & 36.28 & 49.42 & 54.80      & 64.44 & 79.19 & 83.62        & 68.41 & 82.89 & 91.76            \\
Finetune   \cite{guo2020broader}  (RN10)             & 25.97 & 31.32 & 35.49       & 48.11 & 59.31 & 66.48     & 79.08 & 87.64 & 90.89        & 89.25 & 95.51 & 97.68            \\
CHEF  \cite{adler2021crossdomain}    (RN10)    & 24.72 & 29.71 & 31.25       & 41.26 & 54.30  & 60.86     & 74.15 & 83.31 & 86.55        & 86.87 & 94.78 & 96.77            \\
STARTUP \cite{phoo2021selftraining}    (RN10) & 26.94 & 33.19 & 36.91       & 47.22 & 58.63 & 64.16     & 82.29 & 89.26 & 91.99        & 93.02 & 97.51 & 98.45            \\
%ConFeSS                 & 27.09 & 33.57 & 39.02       & 48.85 & 60.1  & 65.34     & 84.65 & 90.4  & 92.66        & 88.88 & 95.34 & 97.56            \\ 
DeepCluster2 \cite{caron2020swav,ericsson2020well} (IN1K, RN50)& 26.51 & 31.51 & 34.17 & 40.73 & 49.91 & 53.65 & 88.39 & 92.02 & 93.07 & 93.63 & 96.63 & 97.04\\
\hline
P$>$M$>$F (DINO/IN1K, ResNet50) & 27.13 &	31.57 &	34.17 &	43.78 &	54.06 &	57.86 &	\textbf{89.18} &	\textbf{93.08} & \textbf{96.06} &	\textbf{95.06} &	97.25 &	97.77 \\
P$>$M$>$F (DINO/IN1K, ViT-small) & \textbf{27.27} & \textbf{35.33} & \textbf{41.39}       & \textbf{50.12} & \textbf{65.78} & \textbf{73.50}      & {85.98} & {91.32} & 95.40         & {92.96} & \textbf{98.12} & \textbf{99.24}           \\
\hline
\end{tabular}
} %< \resizebox
\caption{
% 
\textbf{Broader study of cross-domain few-shot learning} -- Comparison with SOTA FSL algorithms.
% 
}\label{tab:cdfsl}
\end{table*}

==> tab/md_full.tex <==
\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{l|llllllll|ll|l} 
\hline
\multirow{2}{*}{8 in-domain datasets} & \multicolumn{8}{c|}{In-domain}                                                                                & \multicolumn{2}{c|}{Out-of-domain} &         \\ 
\cline{2-12}
                                      & INet                           & Omglot & Acraft & CUB   & DTD   & QDraw & Fungi & Flower                     & Sign  & COCO                    & Avg     \\ 
\hline
ProtoNet \cite{triantafillou2019meta}  (RN18)                      & 67.01                          & 44.5   & 79.56  & 71.14 & 67.01 & 65.18 & 64.88 & 40.26                      & 86.85 & 46.48                   & 63.29  \\
CNAPs  \cite{requeima2020fast}  (RN18+Adapter)                           & 50.8                           & 91.7   & 83.7   & 73.6  & 59.5  & 74.7  & 50.2  & 88.9                       & 56.5  & 39.4                    & 66.90    \\ %(50.8 + 91.7 + 83.7 + 73.6 + 59.5 + 74.7 + 50.2 + 88.9 + 56.5 + 39.4)/10=66.9
%\doublecheck{SUR} \cite{dvornik2020selecting}   (RN18+Adapter)               & 57.2                           & 93.2   & 84.6   & 70.6  & \doublecheck{71}   & 81.3  & 64.2  & 82.8                       & 53.4  & 50.1                    & 70.72   \\
{SUR} \cite{dvornik2020selecting}   (RN18+Adapter)               & 57.2                           & 93.2   & \textbf{90.1}   & 82.3  & 73.5   & 81.9  & 67.9  & 88.4                       & 67.4  & 51.3                    & 75.32  \\ %(57.2 + 93.2 + 90.1 + 82.3 + 73.5 + 81.9 + 67.9 + 88.4 + 67.4 + 51.3)/10=75.32
%SimpleCNAPS \cite{Bateni_2020_CVPR}                      & 56.5                           & 91.9   & 83.8   & 76.1  & 70    & 78.3  & 49.1  & 91.3                       & 59.2  & 42.4                    & 69.86   \\
%Trans. CNAPS \cite{bateni2020enhancing}                        & 57.9                           & 94.3   & 84.7   & 78.8  & 66.2  & 77.9  & 48.9  & 92.3                       & 59.7  & 42.5                    & 70.32   \\
T-SCNAPs \cite{bateni2020enhancing}  (RN18+Adapter)    & 58.8                           & 93.9   & 84.1   & 76.8  & 69.0  & 78.6  & 48.8  & 91.6  & 76.1  & 48.7                    & 72.64   \\ %(58.8 + 93.9 + 84.1+ 76.8  + 69.0  + 78.6  + 48.8 + 91.6  + 76.1  + 48.7)/10=72.64
URT \cite{liu2020universal}      (RN18+Adapter)         & 55.7                           & 94.4   & 85.8   & 76.3  & 71.8  & 82.5  & 63.5  & 88.2                       & 69.4  & 52.2                    & 73.98  \\ %(55.7+  94.4 + 85.8  + 76.3  + 71.8  + 82.5  + 63.5  + 88.2   + 69.4  + 52.2)/10=73.98
FLUTE \cite{triantafillou2021learning}   (RN18)    & 51.8                           & 93.2   & 87.2   & 79.2  & 68.8  & 79.5  & 58.1  & 91.6                       & 58.4  & 50.0                      & 71.78   \\
URL \cite{li2021universal}  (RN18+Adapter)      & 57.51                          & 94.51  & 88.59  & 80.54 & 76.17 & 81.94 & 68.75 & 92.11                      & 63.34 & 54.03                   & 75.75  \\
ITA \cite{li2021improvingFSL}      (RN18+Adapter)                         & 57.35                          & \textbf{94.96}  & 89.33  & 81.42 & 76.74 & \textbf{82.01} & 67.4  & 92.18                      & 83.55 & 55.75                   & 78.07  \\ 
\hline
P$>$M$>$F (DINO/IN1K, RN50)                 & 67.51                          & 85.91  & 80.3   & 81.67 & \textbf{87.08} & 72.84 & 60.03 & 94.69                      & 87.17 & 58.92                   & 77.61  \\
P$>$M$>$F (DINO/IN1K, ViT-small)               & 74.59                          & 91.79  & 88.33  & 91.02 & 86.61 & 79.23 & 74.2  & 94.12                      & 88.85 & 62.59                   & 83.13  \\
P$>$M$>$F (DINO/IN1K, ViT-base)               & \textbf{77.02}                          & 91.76  & {89.73}  & \textbf{92.94} & 86.94 & 80.2  & \textbf{78.28} & \textbf{95.79}                      & \textbf{89.86} & \textbf{64.97}                   & \textbf{84.75}  \\
%BEiT (sup21k) + PN + FT (ViT-bs)      & 81.96                          & 94.19  & 91.62  & 93.76 & 84.97 & 83.48 & 81.76 & 98.84                      & 91.29 & 65.09                   & 86.696  \\ 
\hline
\multirow{2}{*}{In-domain = ImageNet} & \multicolumn{1}{c|}{In-domain} & \multicolumn{9}{c|}{Out-of-domain}                                                                                &         \\ 
\cline{2-12}
                                      & \multicolumn{1}{c|}{INet}      & Omglot & Acraft & CUB   & DTD   & QDraw & Fungi & \multicolumn{1}{c}{Flower} & Sign  & COCO                    & Avg     \\ 
\hline
ProtoNet \cite{triantafillou2019meta} (RN18)                       & \multicolumn{1}{l|}{50.5}      & 59.98  & 53.1   & 68.79 & 66.56 & 48.96 & 39.71 & \multicolumn{1}{l}{85.27}  & 47.12 & 41                      & 56.10  \\
ALFA+FP-MAML \cite{baik2020metalearning} (RN12)   & \multicolumn{1}{l|}{52.8}      & 61.87  & 63.43  & 69.75 & 70.78 & 59.17 & 41.49 & \multicolumn{1}{l}{85.96}  & 60.78 & 48.11                   & 61.41  \\
BOHB \cite{saikia2020optimized}  (RN18)      & \multicolumn{1}{l|}{51.92}     & 67.57  & 54.12  & 70.69 & 68.34 & 50.33 & 41.38 & \multicolumn{1}{l}{87.34}  & 51.8  & 48.03                   & 59.15  \\
CTX \cite{doersch2020crosstransformers}  (RN34)  & \multicolumn{1}{l|}{62.76}     & 82.21  & 79.49  & 80.63 & 75.57 & 72.68 & 51.58 & \multicolumn{1}{l}{\textbf{95.34}}  & 82.65 & 59.9                    & 74.28  \\ 
\hline
P$>$M$>$F (DINO/IN1K, RN50)                 & \multicolumn{1}{l|}{67.08}     & 75.33  & 75.39  & 72.08 & 86.42 & 66.79 & 50.53 & \multicolumn{1}{l}{94.14}  & 86.54 & 58.2                    & 73.25   \\
P$>$M$>$F (DINO/IN1K, ViT-small)               & \multicolumn{1}{l|}{74.69}     & 80.68  & 76.78  & 85.04 & 86.63 & 71.25 & 54.78 & \multicolumn{1}{l}{94.57}  & 88.33 & 62.57                   & 77.53  \\
P$>$M$>$F (DINO/IN1K, ViT-base)               & \multicolumn{1}{l|}{\textbf{76.69}}     & \textbf{81.42}  & \textbf{80.33}  & \textbf{84.38} & \textbf{86.87} & \textbf{75.43} & \textbf{55.93} & \multicolumn{1}{l}{95.14}  & \textbf{89.68} & \textbf{65.01}                   & \textbf{79.09}  \\
%BEiT (sup21k) + PN + FT (ViT-bs)      & \multicolumn{1}{l|}{84.39}     & 79.58  & 81.51  & 95.66 & 86.14 & 76.85 & 64.25 & \multicolumn{1}{l}{99.19}  & 91.56 & 69.91                   & 82.904  \\
\hline
\end{tabular}
} %< \resizebox
\caption{
\textbf{Meta-Dataset} -- Comparison with SOTA FSL algorithms.
}\label{tab:metadataset}
\end{table*}

==> tab/single_domain.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line

\begin{tabular}{l|cc|l|l|l|l} 
\hline
\multirow{2}{*}{Method (Backbone)} & Ext. & Ext. & \multicolumn{2}{l|}{CIFAR-FS} & \multicolumn{2}{l}{MiniImageNet}  \\ 
\cline{4-7}
& dat. & lab.  & 5w1s  & 5w5s  & 5w1s  & 5w5s \\ 
\hline
\textbf{Inductive} &&&&&\\
ProtoNet (CNN-4-64) \cite{snell2017prototypical} && & 49.4 & 68.2 & 55.5 & 72.0 \\
Baseline++ (CNN-4-64) \cite{chen2019closerLook} & & & & & 48.2 & 66.4 \\
MetaOpt-SVM (ResNet12) \cite{lee2019meta}     &        &                               & 72.0    & 84.3       & 61.4  & 77.9 \\
%ProtoNet + MABAS (ResNet12) & & 65.1 & 82.7 & 73.5 & 85.5 \\
Meta-Baseline (ResNet12) \cite{chen2021metaBaseline} & & &  &  & 68.6 & 83.7 \\ 
RS-FSL (ResNet12) \cite{afham2021rich} & & \ding{51}               &       &                   & 65.3  &  \\
\textbf{Transductive} &&&&&\\
Fine-tuning (WRN-28-10) \cite{dhillon2020baselineFSL} & & & 76.6 & 85.8 & 65.7 & 78.4 \\
SIB (WRN-28-10) \cite{Hu2020Empirical}     &&                               & 80.0    & 85.3            & 70.0    & 79.2 \\
PT-MAP (WRN-28-10) \cite{hu2021leveraging}            & &                    & \textbf{87.7} & 90.7      & 82.9 & 88.8 \\
%Illu-Aug (WRN-28-10) \cite{zhang2021sill}      &       &                    & \textbf{87.7} & 91.1      & 83.0 & 89.1 \\
CNAPS + FETI (ResNet18) \cite{bateni2020enhancing} & \ding{51}  & \ding{51}               &       &                   & 79.9  & 91.5 \\
\textbf{Self-supervised} &&&&&\\
%MoCo (ResNet50) \cite{tian2020rethinking} & \ding{51} & & & & 54.2 & 73.0 \\
ProtoNet (WRN-28-10) \cite{gidaris2019boosting} &&                               & 73.6  & 86.1              & 62.9  & 79.9 \\
ProtoNet (AMDIM ResNet) \cite{chen2021selfsupervised} & \ding{51} & & &  & 76.8 & 91.0 \\
EPNet + SSL (WRN-28-10) \cite{rodriguez2020embedding} & \ding{51} && & & 79.2 & 88.1 \\
\textbf{Semi-supervised} &&&&&\\
LST (ResNet12) \cite{li2019learning} & \ding{51} & & & & 70.1 & 78.7 \\
%LST fully-sup. (ResNet12) \cite{li2019learning} & \ding{51} & \ding{51} & & & 80.4 & 83.3 \\
PLCM (ResNet12) \cite{huang2021lossConfSSLFSL} & \ding{51} & & 77.6 & 86.1 & 70.1 & 83.7 \\
\hline
P$>$M$>$F (IN1K, RN50)                              & \ding{51}    &                 & 73.7  & 84.0                  & 79.2  & 92.0 \\ 
P$>$M$>$F (IN1K, ViT-Small)                           & \ding{51}  &                   & 81.1  & \textbf{92.5}                  & 93.1  & 98.0 \\
P$>$M$>$F (IN1K, ViT-base)                               & \ding{51}   &                  & 84.3  & {92.2}         & \textbf{95.3}  & \textbf{98.4} \\
\hline
\end{tabular}

} % \resizebox
\caption{
\textbf{miniImageNet \& CIFAR} -- Comparison with representative SOTA FSL algorithms. Methods using external data and/or labels are indicated. 
} % \caption
\label{tab:single}
\end{table}
